Memory-aware Scheduling for Complex Wired Networks with Iterative Graph Optimization

Memory-aware network scheduling is becoming increasingly important for deep neural network (DNN) inference on resource-constrained devices. However, due to the complex cell-level and network-level topologies, memory-aware scheduling becomes very challenging. While previous algorithms all suffer from poor scalability, in this paper, we propose an efficient memory-aware scheduling framework based on iterative computation graph optimization. Our framework features an iterative graph fusion algorithm that simplifies the computation graph while preserving the scheduling optimality. We further propose an integer linear programming formulation together with topology-aware variable pruning to schedule the simplified graph efficiently. We evaluate our method against prior-art algorithms on different networks and demonstrate that our method outperforms existing techniques in all the benchmarks, reducing the peak memory footprint by 13.4%, and achieving better scalability for networks with complex network-level topologies.

==> docs/outline.tex <==
\section*{Outline}
\begin{itemize}
    \item To democratize AI, there is an increasing demand to deploy deep neural networks (DNNs) on resource constrained edge devices with limited compute and memory. In contrast, DNN topology is getting more and more complex: on one hand, networks optimized by neural architecture search (NAS), e.g., NASNet, DARTS, RandWire, etc, comprise of complex and irregular wire connections; on the other hand, multi-scale networks, e.g., HRNet, BiFPN, etc, introduce parallel branches and cross-resolution fusions for multi-scale feature extraction. Network scheduling, which determines the execution order for each operator in the computation graph, becomes very important as it directly affect the activation memory footprint during inference and hence, whether the network can execute on the device or not. \ml{Need a figure on RandWire/NASNet Cell and HRNet-Arch.}
    \item Though important, the memory-aware scheduling problem is very challenging due to the huge schedule space. First, NAS tends to generate complex cells with more operators compared to hand-designed cells. For example, NASNet cells have 10 operators per cell while RandWire cells have almost 100 operators. In contrast, ResNet and MobileNetV2 blocks only have 2 or 3 operators. Meanwhile, while traditional networks leverage a linear topology to connect the basic cells head-to-tail in sequence, recent models, including HRNet, ScaleNAS, BiFPN, etc, introduce much more complex network topologies with parallel branches and cross-scale fusions. The large number of operators and the complex network topologies significantly increase the problem scale.
    \item Existing deep learning frameworks, including Tensorflow, TVM, etc, are unaware of the memory footprint and use simple topology-based scheduling strategy. Serenity is the first systematic study of the memory-constrained scheduling problem and proposes an approximate dynamic programming (DP)-based algorithm to determine the operator execution order and reduces the peak memory footprint. HMCOS further proposes a hierarchical approach which leverages hierarchical computation graph to simplify the network structure and iteratively disassemble the graph for scheduling. Though both Serenity and HMCOS demonstrate promising results, they suffer from the following key problems:
    \begin{itemize}
        \item Relies on extra memory budget parameters for scheduling space pruning.
        \item Ignores the multi-scale networks, for which graph partitioning cannot be easily applied without compromising the solution optimality.
        \item Heuristic based methods: Serenity relies on approximation in DP to prune the optimization space while HMCOS relies on grouping and disassembling. The impact of these methods on the scheduling quality hence is hard to estimate. 
    \end{itemize}
    \item Contributions:
    \begin{itemize}
        \item Propose an MILP formulation for network scheduling with optimal memory footprint.
        \item Propose a series of techniques to speedup solving MILP while maintaining the optimality of the solution
        \item Compared to previous methods, achieve both better scheduling quality and less scheduling time.
    \end{itemize}
    \item Preliminaries:
    \begin{itemize}
        \item Definition 1: computation graph $G(V, E)$
        \item Definition 2: operator stable and transient footprint
        \item Definition 3: network scheduling and memory footprint w.r.t a schedule
    \end{itemize}
    \item Main methods:
    \begin{itemize}
        \item Understanding the runtime bottleneck for network scheduling: compare parallel structures and linear structures
        \item MILP formulation
        \item Topology-aware solution space pruning
        \item Operator fusion: \ml{for each fusion strategy, need formal definition of the conditions and formal proof of the solution optimality.}
        \begin{itemize}
            \item Linear vertices fusion: 
            \begin{itemize}
                \item Condition 1: inplace or logical operators, e.g., BN, ReLU, squeeze/unsqueeze, etc
                \item Condition 2: blocks with decreasing transient memory footprint
            \end{itemize}
            \item Generalized residual blocks fusion
        \end{itemize}
    \end{itemize}
    \item Experimental results:
    \begin{itemize}
        \item Point out for networks with linear topologies, we leverage the network partitioning algorithm proposed in Serenity.
        \item Peak memory footprint and scheduling time comparison with prior-art methods, including RPO, Serenity, HMCOS (key results).
        \item Ablation study: use NASNet and HRNet-W18-Small-V1 as an example and show the impact of the proposed speedup techniques on 1) MILP problem size, 2) scheduling time, and 3) final results.
        \item Ablation study: a scalability comparison with HMCOS. Gradually increase the size of the RandWire benchmark and compare the problem size as well as the latency.
    \end{itemize}
\end{itemize}

\begin{table}[h]
\caption{Peak memory footprint comparison with prior art methods.}
\label{table:mem_footprint_comp}
\begin{tabular}{c|ccccc}
\hline \hline
                   & RPO & Serenity & HMCOS & Ours & Improvement \\
\hline
NASNet-A           &     &          &       &      &             \\
AmoebaNet-A        &     &          &       &      &             \\
DARTS              &     &          &       &      &             \\
RandWire 1         &     &          &       &      &             \\
RandWire 2         &     &          &       &      &             \\
RandWire 3         &     &          &       &      &             \\
HRNet-W18-Small-V1 &     &          &       &      &             \\
HRNet-W18-Small-V2 &     &          &       &      &             \\
HRNet-W18          &     &          &       &      &             \\
\hline 
Average            &     &          &       &      &             \\          
\hline \hline
\end{tabular}
\end{table}


\begin{table}[h]
\caption{Scheduling time comparison with prior art methods.}
\label{table:mem_footprint_comp}
\begin{tabular}{c|ccc}
\hline \hline
                   & HMCOS & Ours & Speedup     \\
\hline
NASNet-A           &       &      &             \\
AmoebaNet-A        &       &      &             \\
DARTS              &       &      &             \\
RandWire 1         &61       &2.4      &             \\
RandWire 2         &       &0.2      &             \\
RandWire 3         &472       &65      &             \\
HRNet-W18-Small-V1 &       &      &             \\
HRNet-W18-Small-V2 &       &      &             \\
HRNet-W18          &       &      &             \\
\hline 
Average            &       &      &             \\          
\hline \hline
\end{tabular}
\end{table}


